A novel agent with formal goal-reaching guarantees: an experimental study with a mobile robot

Reinforcement Learning (RL) has been shown to be effective and convenient for a number of tasks in robotics. However, it requires the exploration of a sufficiently large number of state-action pairs, many of which may be unsafe or unimportant. For instance, online model-free learning can be hazardous and inefficient in the absence of guarantees that a certain set of desired states will be reached during an episode. An increasingly common approach to address safety involves the addition of a shielding system that constrains the RL actions to a safe set of actions. In turn, a difficulty for such frameworks is how to effectively couple RL with the shielding system to make sure the exploration is not excessively restricted. This work presents a novel safe model-free RL agent called Critic As Lyapunov Function (CALF) and showcases how CALF can be used to improve upon control baselines in robotics in an efficient and convenient fashion while ensuring guarantees of stable goal reaching. The latter is a crucial part of safety, as seen generally. With CALF all state-action pairs remain explorable and yet reaching of desired goal states is formally guaranteed. Formal analysis is provided that shows the goal stabilization-ensuring properties of CALF and a set of real-world and numerical experiments with a non-holonomic wheeled mobile robot (WMR) TurtleBot3 Burger confirmed the superiority of CALF over such a well-established RL agent as proximal policy optimization (PPO), and a modified version of SARSA in a few-episode setting in terms of attained total cost.

==> input/intro.tex <==
Reinforcement learning is a control philosophy where, unlike the classical theory, the controller is learned (adapted) through the pure \textit{experience} \ie data generated from the system in some manner: via exploring a predefined region of the state space (so called \textit{tabular methods}), Monte-Carlo runs or even online \cite{Sutton2018ReinforcementL,Bertsekas2019Reinforcementl,Lewis2013Reinforcementl,Vrabie2012OptimalAdaptiv,Bouzy2006MonteCarloGo,Lazaric2007Reinforcementl,Vodopivec2017montecarlotre}.
Its applications range from robotics \cite{Kumar2016Optimalcontrol,Borno2013TrajectoryOpti,Tassa2012Synthesisstabi,Surmann2020DeepReinforcem,Akkaya2019Solvingrubiks} to games such as Go, chess, shogi (also known as Japanese chess) \cite{Silver2016Masteringgame,Silver2018generalreinfor}, and even complex video games such as StarCraft II \cite{Vinyals2019Grandmasterlev}.
Some variants of simple policy gradients \cite{Baxter2001Infinitehorizo,Kakade2001naturalpolicy,Peters2006Policygradient}, like REINFORCE, do not utilize practically anything from the classical control theory and are more akin to stochastic approximation, which is common in pure data science.
Other, more intricate methods use the so called actor-critic structure, which is much closer to control.
Actor manifests the controller itself, whereas the critic can be interpreted as a controller adaptation unit.
Nowadays, the actor and critic are usually implemented as neural nets.
Evidently, it is crucial to study how the net weights converge.
Results in this direction are numerous.
But, and what is more important from the control field standpoint, the closed-loop stability only relatively recently has been starting to attract attention.
We point out in this note that the closed-loop stability is crucial not only by itself, but it also affects the controller adaptation manifested by the critic.
%Attempts to guarantee stability under reinforcement learning were and are being made.
One research direction to guarantee stability under reinforcement learning uses the techniques of classical adaptive control, robustifying controls in particular.
The contribution of this work if two-fold: first, we indicate and study in a simulation the limitations of robustifying controls in reinforcement learning.
This should be taken into account by the researchers in stabilizing reinforcement learning taking the route of adaptive control.
Second, we provide a new stochastic analysis of the critic net convergence and point out at the role of the environment stability in it.
%We start first with an overview of stabilizing reinforcement learning.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{On stabilizing reinforcement learning}
\label{sub_stabrl}

Three general groups of approaches to stabilizing reinforcement learning can be formulated: shield-based reinforcement learning, fusion of model-predictive control and reinforcement learning and Lyapunov-based reinforcement learning.
% In this section we will overview these approaches and compare them to the proposed method. 
The first group of approaches suggests to directly discard unsafe actions via, generally speaking, a filter which, depending on the context, may be called a shield, an overseer, a supervisor etc.
These algorithms vary in the way of how exactly the shield checks actions for safety and issues an emergency solution.

The actual design of the shield may be as simple as human-based \ie manual \cite{Saunders2017TrialerrorTow}, or as complex as formal-logic based \cite{Tan2020DeductiveStabi,Platzer2008Keymaerahybrid,Platzer2009EuropeanTrain,Fulton2018Safereinforcem}.
Fusion with model-predictive control is active subfield in stabilizing reinforcement learning (see \eg \cite{Zanon2020SafeReinforcem,Zanon2019Practicalreinf,Zanon2022Stabilityconst,Koller2018LearningBased,Berkenkamp2017SafeModelbase,Berkenkamp2019Safeexploratio}).
It is no wonder since model-predictive control possesses such an established machinery for guaranteeing stability of the closed loop, such as terminal costs, terminal constraints, contraction tools etc.
Finally, the Lyapunov stability theory was recognized in reinforcement learning already by Perkins \& Barto \cite{Perkins2002LyapunovDesign,Perkins2001Lyapunovconstr}.
Advancements were made since \cite{Chow2018Lyapunovbased,Berkenkamp2017SafeModelbase}, although such approaches to stabilizing reinforcement learning were offline and required checking a Lyapunov decay property over a region in the state space during running the agent.
This is not always feasible in industrial applications, such as robotics.
To this Lyapunov-based stabilizing reinforcement learning, agent design based on stabilization techniques of adaptive control can be categorized (approaches can be traced back to the early 2010s \eg \cite{Zhang2011Datadrivenrob}).

An elaborate approach was suggested by \cite{vamvoudakis2015asymptotically}, whose elements found application in later works \eg \cite{Yang2019Provablyglobal,Wei2020DiscreteTimeI,Su2020DecentralizedE,Zhang2020RobustOptimal,Jha2019InitialExcitat,Kontoudis2019KinodynamicMot,Jha2018DirectAdaptivea,Luy2018Machinelearnin,Yang2020Safeintermitte,Shi2023SafeReinforcem}, some from the recent years.
The key idea was to use robustifying controls inspired by \cite{Polycarpou2003lineapproximat}.
In the next section, we overview this technique of stabilizing reinforcement learning by robustifying controls.
%Essentially, a Lyapunov function for the closed-loop system was suggested in \cite{vamvoudakis2015asymptotically}, as well as one for the actor's and one for critic's weights, based on the value function utilizing a special \textit{robustifying term} in the agent's policy.
%We give a synopsis of the work \cite{vamvoudakis2015asymptotically} in the next section.
%Then, we indicate a flaw in the respective stability analysis.
%It is stipulated that \cite{vamvoudakis2015asymptotically} erroneously followed the ideas of adaptive control by \cite{polycarpou2003line}.
%Implications for similar control schemes are discussed.

%The authors of \cite{vamvoudakis2015asymptotically} claimed to obtain a Lyapunov function for the closed-loop system, as well as for the actor's and critic's weights, based on the value function utilizing a special \textit{robustifying term} in the agent's policy.

%The work \cite{vamvoudakis2015asymptotically} can be roughly classified as Lyapunov-based stabilizing reinforcement learning and is, moreover, online.
%The authors of \cite{vamvoudakis2015asymptotically} claimed to obtain a Lyapunov function for the closed-loop system, as well as for the actor's and critic's weights, based on the value function utilizing a special \textit{robustifying term} in the agent's policy.
%Unfortunately, the respective mathematical derivations contain a serious flaw.
%We critically analyze it after a synopsis of the work \cite{vamvoudakis2015asymptotically} which we give in the next section.
%It is stipulated that Vamvoudakis et al. erroneously followed the ideas of adaptive control by \cite{polycarpou2003line}.
%In our view, the work \cite{vamvoudakis2015asymptotically} cannot be fixed in any way that could follow the claimed approach closely.
%Nevertheless, it is actively cited: refer \eg to \cite{wei2020ImpulsiveADP, su2020decentralized, zang2020robustNonlinear, Jha2019LTIsystems, KinodynamicVamvoudakis, jha2018LTIwithoutPEcondition, MLbasedMultipleAgentsNguen, YangVamSafe}.
%
%\red{ here} \cite{YangVamSafe} used a robustifying term
%
%Also, similar ideas can be traced back to \cite{zang2011robust}.

==> input/results_old.tex <==
\blue{HERE GOES NEW TEXTBLOCK}

\red{For Pavel: needs polishing!}

\subsection{System description}
We consider a differential drive mobile wheeled robot for testing proposed algorithms. The goal is to achieve autonomous stabilization of the robot at the origin of a coordinate system, starting from non-zero initial conditions. This means the robot must move from an arbitrary starting position to the origin (0,0) on a 2D plane.
In the environment, there is a designated high-cost zone, which could represent a physical obstacle like a swamp, puddle, or any other phenomenon that can adversely impact the robot's movement. 
Within this high-cost zone, the robot's maximum velocity is constrained to 1 cm per second to mitigate potential damage or difficulties in navigation.
	
The differential drive model describes the motion of the wheeled robot. In this model, the robot has two wheels mounted on either side, which can rotate independently. 
The position and orientation of the robot in the plane can be described by the state variables \((x, y, \theta)\), where:
	
	\begin{itemize}
		\item \(x\) and \(y\) represent the coordinates of the robot in the plane.
		\item \(\theta\) is the orientation angle of the robot with respect to a reference direction.
	\end{itemize}
	
The kinematic equations governing the motion of the robot are:
	
\begin{equation}
	\begin{aligned}
		\dot{x} &= v \cos(\theta) \\
		\dot{y} &= v \sin(\theta) \\
		\dot{\theta} &= \omega
	\end{aligned}
\end{equation}

	
where:
\begin{itemize}
	\item \(v\) is the linear velocity of the robot.
	\item \(\omega\) is the angular velocity (rate of change of orientation).
\end{itemize}
	
	
In the high-cost zone, the linear velocity $v$ is restricted such that $v \leq 1 \text{ cm/s}$. 
Outside of this zone, the robot can move at its maximum possible speed, as defined by the algorithm.

The control objective is to design a control law for $v$ and $\omega$ to stabilize the robot at the origin $(0,0)$. 
This involves navigating from any initial position to the origin while respecting the velocity constraints in the high-cost zone.
Experiments are conducted to validate the proposed algorithms under various initial conditions and environments, including the presence of the high-cost zone. 
The performance metrics typically include the time taken to reach the origin, the path taken by the robot, and its behavior in and around the high-cost zone.
\blue{HERE ENDS NEW TEXTBLOCK}

In this section, we investigate the performance of CALF and SARSA-m as the benchmark agent and compare them with a nominal stabilizer, and three MPC agents with different horizons.
The latter are taken to get an idea about a nearly optimal controller for the stated problem.
The code for the environment simulation, CALF, SARSA-m, MPC and nominal stabilizer may be found under \url{https://github.com/osinenkop/rcognita-calf}.

In our studies, we observed that a significant horizon of length 25 was sufficient to fulfill the stated goal.
This controller is further referred to as MPC25.
Notice that MPC25 may lack practicability due to such a long horizon, especially taking into account possible disturbances.
\blue{As the horizon length increases, the number of decision variables and constraints in the optimization problem grows, leading to increased computational complexity. 
Solving this problem within a reasonable time frame becomes more challenging as the horizon extends.
For real-time applications, such as controlling a differential drive mobile robot, the control decisions need to be computed and applied within very short time intervals. 
The extensive computations required for a 25-step horizon can exceed the available computational resources and time, making it impractical for real-time implementation.}
In this regard, CALF and SARSA-m are beneficial as they do not use any models.
Again, MPC25 was rather taken to get a clue of the best possible cost.

\begin{figure}
	\centering
	\includegraphics{gfx/kinematic_model_picture1.pdf}
%	\input{gfx/3wrobot-Cartesian-plane.pdf_tex}
	\caption{Robot kinematics and its frames of interests.}
	\label{fig_3wrobot}
\end{figure}

Now, we get to the optimal control problem.
The base environment is a wheeled mobile robot (WMR) depicted in Fig. \ref{fig_3wrobot}.
At time $t$, the origin of the local coordinate frame (base) of the robot is located at the point $(x_t, y_t)$ of the world coordinate frame. 
The robot's linear velocity $v(t)$ along the axes determines the direction of motion, while the angular velocity $\omega(t)$ determines the rotation (refer to Fig.~\ref{fig_3wrobot}).
% Thus, the input of the system is a vector of two components $u(t) = \begin{bmatrix} v(t) & \omega(t) \end{bmatrix}$.
The state vector $\state \in \mathbb{R}^3$ and the control input vector (action) $\action \in \mathbb{R}^2$ are defined as

\begin{equation}
	\label{eqn_state_action_3wrobot}
	s \coloneqq \begin{bmatrix} x & y & \vartheta \end{bmatrix}^\top, \action \coloneqq \begin{bmatrix} v & \omega \end{bmatrix}^\top.
\end{equation}

The environment state transition map $\transit$ can be obtained via time discretization of the WMR differential equations which read: $\dot x = v \cos \vartheta, \dot y = v \sin \vartheta, \dot \vartheta = \omega$.
For the studied MPC, we used Euler discretization, whereas for CALF and SARSA-m, $\transit$ is not necessary at all.
In our case study, we used the controller sampling time of 100 ms.

The control actions were constrained by $\action_\min$ and $\action_\max$, which are determined by the actuators' capabilities.
We took those constraints matching Robotis TurtleBot3, namely, 0.22 m/s of maximal magnitude of translational and 2.84 rad/s of rotational velocity, respectively.

The control goal is to drive the robot into $\G = \{ \state \in \R^3: \nrm{\state - \state^*} \le \Delta \}$, where the target state $\state^*$ was taken identical with the origin and $\Delta$ is target pose tolerance.

To make the task challenging, we introduced a spot with a high cost on the plane $R^2$, namely, the cost was defined as (we did not penalize the action and only slightly penalized the angle):
\begin{equation}
	\label{eqn_3wrobotcost}
	\cost \left(\state, \action \right) = x^2 + y^2 + 0.1 \vartheta^2 + 10 \cost' \left(x, y \right), 
\end{equation}
where 
\begin{equation}
	\label{eqn_hotspot}
%	\begin{aligned}
	\cost'(x, y) = \frac{1}{2 \pi \sigma_x \sigma_y } \exp \Bigg(- \frac{1}{2} \left( \frac{\Delta x ^2}{\sigma_x ^ 2}  + \frac{\Delta y ^2}{\sigma_y ^ 2} \right) \Bigg),
%	\end{aligned}
\end{equation}
with $\Delta x = x - \mu_x, \Delta_y = y - \mu_y$; $\sigma_x = \sigma_y = 0.1$ being standard deviations in the along-track and cross-track directions, respectively; and $\mu_x = -0.6, \mu_y = -0.5$ being the high cost spot center. 

We now proceed to the description of the nominal stabilizer.
The action components $v, \omega$ were determined based on the polar coordinate representation of the WMR as per \cite{Astolfi1995Exponentialsta}, namely:
\begin{equation}
	\begin{bmatrix}
		\dot{\rho} \\
		\dot{\alpha} \\
		\dot{\beta}
	\end{bmatrix} = \begin{bmatrix}
		\pm \cos {\alpha} & 0 \\
		\mp \frac{\sin{\alpha}}{\rho} & 1 \\
		\pm \frac{\sin{\alpha}}{\rho} & 0
	\end{bmatrix}     \begin{bmatrix}
		\pm v \\
		\omega
	\end{bmatrix},
\end{equation}
where the top sign (plus or minus) holds if $\alpha \in (- \frac \pi 2, \frac \pi 2]$ and the bottom sign holds if $\alpha \in \left(-\pi, -\pi/2 \right]\cup \left(\pi/2, \pi \right]$.
The transformation into the polar coordinates in turn reads:
\begin{align*}
	\rho &= \sqrt{x ^ 2 + y ^ 2},\\
	\alpha &= -\vartheta + \arctan2(y, x),\\
	\beta &= -\vartheta - \alpha.
	\label{eqn_polar}
\end{align*} 

The stabilizer was set as per:
\begin{align}
	v & \la K_{\rho} \rho,\\
	\omega & \la K_{\alpha}\alpha + K_{\beta} \beta,
\end{align}
where $K_{\rho} > 0, K_{\beta} < 0, K_{\alpha} - K_{\rho} > 0$.

\begin{figure*}
	\centering
	\begin{subfigure}[t]{0.46\textwidth}
		\includegraphics[width=\linewidth]{gfx/confidence.pdf}
		\caption{Learning curves depending on the episode \ie environment run number. The clouds represent the 95 \% confidence intervals. The solid lines are median. Model-predictive controllers, as well as the nominal stabilizer, are given for reference.}
		\label{fig_lrcurves}
	\end{subfigure}
	\phantom{---}
	\begin{subfigure}[t]{0.45\textwidth}
		\includegraphics[width=\linewidth]{gfx/time.pdf}
		\caption{Accumulated cost (logarithmic scale) depending on time in the best learning episode. The clouds represent the 95 \% confidence intervals. The solid lines are medians.}
		\label{fig_accumcost}
	\end{subfigure}
	\caption{Learning curves obtained from 25 seeds of random number generator.}
	\label{fig_cost}
\end{figure*}

\begin{figure*}
	\centering
%			\begin{subfigure}[t]{0.32\textwidth}
%				\includegraphics[width=\linewidth]{gfx/traj1.pdf}
%				\caption{The final trajectories provided by the best learning models (according to the final cost metric).}
%				\label{fig:traj1}
%			\end{subfigure}
	\begin{subfigure}[t]{0.45\textwidth}
		\includegraphics[width=\linewidth]{gfx/trajCALF.pdf}
		\label{fig:traj2}
	\end{subfigure}
	\phantom{---}
	\begin{subfigure}[t]{0.465\textwidth}
		\includegraphics[width=\linewidth]{gfx/trajSARSA.pdf}
		\label{fig:traj3}
	\end{subfigure}
\caption{The robot trajectories in best learning episodes over 25 seeds.}
\label{fig_traj}
\end{figure*}

The robot was run for 30 seconds in each episode.
If the target was not reached, we nominally added a cost of 600 to rule out the cases where the robot simply did not drive to the target while also not getting into the ``hot'' spot determined by $\cost'$.
The target area was to 0.2 in radius around the origin (see Fig.~\ref{fig_traj}).
The initial robot pose was set to $\begin{Bmatrix}  -1 & -1 & \pi/2	\end{Bmatrix}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Discussion of results and conclusion}

As can be seen from the results (Fig.~\ref{fig_traj}, Fig.~\ref{fig_cost}), both reinforcement learning  agents outperformed MPC10 and MPC15 (CALF at once and SARSA-m in the final episode).
The controller MPC25 performed best in terms of cost, but it should only be taken as a reference for a potential nearly best performing approach.
It has a significant horizon length which reduces its practicability.
Unlike MPC25, the studied reinforcement learning agents are totally model-free.
Next, CALF also outperformed the nominal controller.
What is remarkable is that both agents were able to detour the ``hot'' spot (notice in Fig.~\ref{fig_traj} how the nominal stabilizer is blind to the spot).
CALF did it in all best learning episodes, whereas SARSA-m succeeded only in a part of those.
It should be repeated here that plain SARSA did not succeed in our case studies at all.
Overall, CALF always succeeded in reaching the target, thanks to its design and Theorem \ref{thm_calfsstab}, and also outperformed the benchmark agent SARSA-m in terms of learning performance.
This validates the initial claim that ensuring online environment stability is not just practicable, but it is also beneficial for episode-to-episode learning.
	

	


==> input/sota_old.tex <==
There are three principal methodologies for stability-ensuring reinforcement learning: shield-based reinforcement learning, the integration of MPC with reinforcement learning, and Lyapunov-based reinforcement learning.

Shield-based approaches involve a protective filter, also referred to as a shield, overseer, or supervisor, designed to prevent undesirable, say, destabilizing actions.
These methods vary in how they evaluate actions and generate safe alternatives.
Shields range from manual human oversight \cite{Saunders2017TrialerrorTow} to sophisticated formal verification variants \cite{Tan2020DeductiveStabi,Platzer2008Keymaerahybrid,Platzer2009EuropeanTrain,Fulton2018Safereinforcem}.
Unlike human operators, formal logic shields are theoretically error-proof, but they require highly specific application development and can be complex, as detailed in \cite{Koenighofer2020Shieldsynthesi}.
Such techniques have been applied in areas such as probabilistic shielding \cite{Koenighofer2020Safereinforcem,Koenighofer2020Shieldsynthesi}, supervisory systems for autonomous vehicles \cite{Isele2018Safereinforcem}, and safe robotic manipulation \cite{Thananjeyan2021RecoveryrlSaf}.
However, human overseers introduce subjective biases and potential errors, and formal logic shields are often difficult to design.

The combination of MPC and reinforcement learning represents an active frontier in the quest for ensuring stability \cite{Zanon2020SafeReinforcem,Zanon2019Practicalreinf,Koller2018LearningBased,Berkenkamp2017SafeModelbase,Berkenkamp2019Safeexploratio,Oh2023QMPCstable}.
Such a fusion takes various forms, sometimes emphasizing model learning and other times focusing on safety constraints \cite{Karnchanachari2020PracticalReinf,Lowrey2018Planonlinelea,Cai2023Energymanageme,Amos2018Differentiable,Hoeller2020DeepValueMode,East2020InfiniteHorizo,Reddy2019LearningHuman,Finn2017Deepvisualfor,Karnchanachari2020PracticalReinf,Asis2020FixedHorizonT}.
The reinforcement learning dreamer is a notable example that adopts the predictive spirit of MPC \cite{Hafner2020DreamControlL,Wu2023DaydreamerWorl}.
Such approaches draw on the MPC's well-established ability to ensure closed-loop stability via techniques like terminal costs and constraints.
Proposals such as the one by Zanon et al. \cite{Zanon2020SafeReinforcem,Zanon2019Practicalreinf} embed robust MPC within reinforcement learning to maintain safety.
Other research emphasizes the predictive control side more heavily \cite{Koller2018LearningBased,Berkenkamp2017SafeModelbase}, building from a safe starting point towards a predictive model while maintaining the option to revert to safe policies when needed.
%MPC integration with reinforcement learning ensures correctness through established safety and stability protocols, yet the intersection of these stability measures with learning presents areas ripe for further investigation, particularly in continuous-time and stochastic environments.

Lyapunov stability theory is well recognized in reinforcement learning, having roots dating back to the work of Perkins and Barto \cite{Perkins2002LyapunovDesign,Perkins2001Lyapunovconstr}, and has seen significant development since \cite{Chow2018Lyapunovbased,Berkenkamp2017SafeModelbase,Jeddi2023Memoryaugmente,Han2020Actorcriticre,Chang2021Stabilizingneu}.
Typically, these approaches are offline and require validation of a Lyapunov decay condition in the state space.
Chow et al. \cite{Chow2018Lyapunovbased}, for instance, developed a safe Bellman operator to ensure Lyapunov compliance, while Berkenkamp et al. \cite{Berkenkamp2017SafeModelbase} used state space segmentation to validate Lyapunov conditions, demanding certain confidence levels in the statistical environment model.
Online Lyapunov-based approaches also exist, often inspired by adaptive control techniques \cite{Zhang2011Datadrivenrob}.
Robustifying controls, a key component introduced by \cite{vamvoudakis2015asymptotically}, may distort the learning unless certain preconditions are met.
Some reviews may be found in \cite{Kamalapurkar2018Reinforcementl,Osinenko2022Reinforcementl}.
Control barrier functions, another safety feature, have been successfully integrated with reinforcement learning, providing enhanced safety capabilities as seen in simulations with bipedal robots \cite{Choi2020Reinforcementl} and in model-free reinforcement learning agents \cite{Cheng2019Endendsafe}.
Stochastic stability theory provides a basis for correctness \cite{Khasminskii2011StochasticStab}, but the current landscape of Lyapunov-based methods often lacks capacity for real-time application without extensive pre-training, and is generally predicated on specific assumptions about environmental dynamics, such as second-order differentiability \cite{Bhasin2013novelactorcri}, linearity \cite{Vamvoudakis2017Qlearningcont}, or global Lipschitz continuity \cite{Vrabie2012OptimalAdaptiv}.

It should be stressed that policy shaping algorithms \eg \cite{Plisnier2023TransferringMu} may be attractive in their similarity to pre-training the agent to boost learning, no online stabilization can be ensured under them.
In contrast to the existing approaches, CALF is online, bringing the interplay of a stabilizer and the agent onto a rigorous footing, thus providing a viable, model-free approach to combining classical control and reinforcement learning.
This is the essence of the current contribution.
